Multi-Modal Reasoning Graph for Scene-Text Based Fine-Grained Image Classification and Retrieval

Scene text instances found in natural images carry explicit semantic information that can provide important cues to solve a wide array of computer vision problems. In this paper, we focus on leveraging multi-modal content in the form of visual and textual cues to tackle the task of fine-grained image classification and retrieval. First, we obtain the text instances from images by employing a text reading system. Then, we combine textual features with salient image regions to exploit the complementary information carried by the two sources. Specifically, we employ a Graph Convolutional Network to perform multi-modal reasoning and obtain relationship-enhanced features by learning a common semantic space between salient objects and text found in an image. By obtaining an enhanced set of visual and textual features, the proposed model greatly outperforms the previous state-of-the-art in two different tasks, fine-grained classification and image retrieval in the Con-Text and Drink Bottle datasets.

==> ablation_table.tex <==
\setlength\tabcolsep{7pt}
\begin{table*}[!htp]
\begin{center}
\begin{tabular}{ccccccc} 
\multicolumn{1}{c}{\textbf{Input}}        & 
% \multicolumn{1}{c}{\textbf{Attn}}        &
\multicolumn{1}{c}{\textbf{MMR}}& \multicolumn{1}{c}{\textbf{Projection}} & \multicolumn{1}{c}{\textbf{Late Fusion}} & \multicolumn{1}{c}{\textbf{Context}} & \multicolumn{1}{c}{\textbf{Bottles}} \\ \hline
 $G_f$                  & -        & -                                       & -                                        & 62.11                                       & 65.15                                     \\
 $G_{fa}$          & -           & -                                       & -                                        & 63.70                                       & 66.56                                     \\
 $G_{fa}$ + V   &    -       & Avg Pooling                                    & Concat                                   & 70.48                                       & 73.21                                     \\
 $G_{fa}$ + V + T  &  -         & Avg Pooling                                    & Concat                                   & 78.72                                       & 76.43                                     \\
 $G_{fa}$   &    V  & Avg Pooling                                    & Concat                                   & 72.88                                       & 74.96                                     \\
 $G_{fa}$ + T   &    V & Avg Pooling                                   & Concat                                   & 82.51                                       & 77.46                                     \\
 $G_{fa}$    &    V+T & Avg Pooling                                    & Concat                                   & 84.92                                       & 79.31                                     \\

 $G_{fa}$    &   V+T & Attention                               & Concat                                   & 80.39                                       & 78.15                                     \\
 $G_{fa}$    &    V+T & Attention                               & Hadamard                                 & 80.62                                       & 78.23        \\

 $G_{fa}$    &    V+T & GRU                                     & Concat                                   & 83.32                                       & 78.28                                                                 \\
 $G_{fa}$    &    V+T & GRU                                     & Hadamard                                 & 83.44                                       & 78.05                                     \\
 $G_{fa}$    &    V+T & Avg Pooling                                    & MLB~\cite{kim2016hadamard}                                     & 84.51                                       & 78.55                                     \\
 $G_{fa}$    &    V+T & Avg Pooling                                    & Block~\cite{ben2019block}                                  & 85.02                                       & 77.68   
\\

 $G_{fa}$    &    V+T+BBox & Avg Pooling                                    & Hadamard                                    & \boldmath$86.15$                                       & $79.38$
\\\hline
 $G_{fa}$  &    \textbf{V+T+BBox}      & \textbf{Avg Pooling}                                    & \textbf{Concat}                                 & 85.81                                        & \boldmath$79.87$                                    
\end{tabular}
\end{center}
\captionsetup{justification=centering}
\caption{Results obtained on each incremental step of our model. \textit{Input} depicts the features that the model is using that are not an input to the multi-modal reasoning module (MMR). \textit{MMR} refers to the features being used by itself. \textit{Projection} is the method used to reduce the dimensionality of the output coming from the MMR as ${V_G}$. \textit{Late Fusion} showcases the method employed to combine the features coming from $V_{Gf}$ and $G_{fa}$. Results are shown in terms of the mAP(\%).}
\label{tab:quantitative_res}
\end{table*}

==> ablation_tablev2.tex <==
\setlength\tabcolsep{7pt}
\begin{table*}[!htp]
\begin{center}
\small

\begin{tabular}{cccc|cc|ccc|cc|cc}
\multicolumn{4}{c|}{\textbf{Input Features}}                     & \multicolumn{2}{c|}{\textbf{Global Enc.}} & \multicolumn{3}{c|}{\textbf{MMR}}              & \multirow{2}{*}{\textbf{Projection}} & \multirow{2}{*}{\textbf{Late Fusion}} & \multirow{2}{*}{\textbf{Context}} & \multirow{2}{*}{\textbf{Bottles}} \\
\textbf{Global} & \textbf{Local} & \textbf{Text} & \textbf{Bbox} & \textbf{Gf}      & \textbf{Attn.}     & \textbf{Vf} & \textbf{Tf} & \textbf{Pos. Enc.} &                                      &                                       &                                   &                                   \\ \hline
y               & \xmark              & x             & x             & Y                & x                      & x           & x           & x                  & -                                    & -                                     & 62.11                             & 65.15                             \\
y               & x              & x             & x             & y                & y                      & x           & x           & x                  & -                                    & -                                     & 63.70                             & 66.56                             \\
y               & y              & x             & x             & y                & y                      & x           & x           & x                  & Avg Pooling                          & Concat                                & 70.48                             & 73.21                             \\
y               & y              & x             & x             & y                & y                      & y           & x           & x                  & Avg Pooling                          & Concat                                & 72.88                             & 74.96                             \\
y               & y              & y             & x             & y                & y                      & x           & x           & x                  & Avg Pooling                          & Concat                                & 78.72                             & 76.43                             \\
y               & y              & y             & x             & y                & y                      & y           & x           & x                  & Avg Pooling                          & Concat                                & 82.51                             & 77.46                             \\
y               & y              & y             & x             & y                & y                      & y           & y           & x                  & Avg Pooling                          & Concat                                & 84.92                             & 79.31                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & Avg Pooling                          & Concat                                & 85.81                             & 79.87                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & Avg Pooling                          & MLB                                   & 84.23                             & 78.56                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & Avg Pooling                          & Block                                 & 85.11                             & 79.15                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & Attention                            & Concat                                & 81.09                             & 78.45                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & Attention                            & MLB                                   & 80.83                             & 78.26                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & Attention                            & Block                                 & 80.82                             & 78.42                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & GRU                                  & Concat                                & 83.93                             & 78.89                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & GRU                                  & MLB                                   & 83.12                             & 78.21                             \\
y               & y              & y             & y             & y                & y                      & y           & y           & y                  & GRU                                  & Block                                 & 83.80                             & 78.74                            
\end{tabular}

\end{center}
\captionsetup{justification=centering}
\caption{Results obtained on each incremental step of our model. \textit{Input} depicts the features that the model is using that are not an input to the multi-modal reasoning module (MMR). \textit{MMR} refers to the features being used by itself. \textit{Projection} is the method used to reduce the dimensionality of the output coming from the MMR as ${V_G}$. \textit{Late Fusion} showcases the method employ to combine the features coming from $V_{Gf}$ and $G_{fa}$. Results are shown in terms of the mAP(\%).}
\label{tab:quantitative_res}
\end{table*}

==> quantitative_table_BKP.tex <==
\setlength\tabcolsep{7pt}
\begin{table*}[!htp]
\begin{center}
\small
\begin{tabular}{l|cccc}
\textbf{Model}                 & \multicolumn{1}{l}{\textbf{Projection}} & \multicolumn{1}{l}{\textbf{Late Fusion}} & \multicolumn{1}{l}{\textbf{Con-Text}} & \multicolumn{1}{l}{\textbf{Bottles}} \\ \hline
CNN                            & -                                       & -                                        & 62.11                                       & 65.15                                     \\
CNN+Attn                       & -                                       & -                                        & 63.70                                       & 66.56                                     \\
CNN+Attn+Local Feats           & Avg Pooling                                    & Concat                                   & 70.48                                       & 73.21                                     \\
CNN+Attn+Local Feats + Text           & Avg Pooling                                    & Concat                                   & 78.72                                       & 76.43                                     \\
CNN+Attn+MMR(Local Feats)      & Avg Pooling                                    & Concat                                   & 72.88                                       & 74.96                                     \\
CNN+Attn+MMR(Local Feats)+Text & Avg Pooling                                   & Concat                                   & 82.51                                       & 77.46                                     \\
CNN+Attn+MMR(Local Feats+Text) & Avg Pooling                                    & Concat                                   & 84.92                                       & 79.31                                     \\

CNN+Attn+MMR(Local Feats+Text) & Attention                               & Concat                                   & 80.39                                       & 78.15                                     \\
CNN+Attn+MMR(Local Feats+Text) & Attention                               & Hadamard                                 & 80.62                                       & 78.23        \\

CNN+Attn+MMR(Local Feats+Text) & GRU                                     & Concat                                   & 83.32                                       & 78.28                                                                 \\
CNN+Attn+MMR(Local Feats+Text) & GRU                                     & Hadamard                                 & 83.44                                       & 78.05                                     \\
CNN+Attn+MMR(Local Feats+Text) & Avg Pooling                                    & MLB                                      & 84.51                                       & 78.55                                     \\
CNN+Attn+MMR(Local Feats+Text) & Avg Pooling                                    & Block                                    & 85.02                                       & 77.68   
\\

Previous + Positional Encoder & Avg Pooling                                    & Hadamard                                    & \boldmath$86.15$                                       & $79.38$
\\\hline
\textbf{Final Model}      & \textbf{Avg Pooling}                                    & \textbf{Concat}                                 & 85.81                                        & \boldmath$79.87$                                    
\end{tabular}
\end{center}
\captionsetup{justification=centering}
\caption{Ablation studies and results obtained on each incremental step of the proposed model. \textit{Projection} refers to the method used to reduce the dimensionality of the output coming from the MMR as ${Gf}$. \textit{Late Fusion} showcases the method employed to combine the features coming from $V_{Gf}$ and $G_{fa}$. All results are depicted in terms of the mAP(\%).}
\label{tab:quantitative_res}
\end{table*}
